Learning by Analogy: Diverse Questions Generation in Math Word Problem

Solving math word problem (MWP) with AI techniques has recently made great progress with the success of deep neural networks (DNN), but it is far from being solved. We argue that the ability of learning by analogy is essential for an MWP solver to better understand same problems which may typically be formulated in diverse ways. However most existing works exploit the shortcut learning to train MWP solvers simply based on samples with a single question. In lack of diverse questions, these methods merely learn shallow heuristics. In this paper, we make a first attempt to solve MWPs by generating diverse yet consistent questions/equations. Given a typical MWP including the scenario description, question, and equation (i.e., answer), we first generate multiple consistent equations via a group of heuristic rules. We then feed them to a question generator together with the scenario to obtain the corresponding diverse questions, forming a new MWP with a variety of questions and equations. Finally we engage a data filter to remove those unreasonable MWPs, keeping the high-quality augmented ones. To evaluate the ability of learning by analogy for an MWP solver, we generate a new MWP dataset (called DiverseMath23K) with diverse questions by extending the current benchmark Math23K. Extensive experimental results demonstrate that our proposed method can generate high-quality diverse questions with corresponding equations, further leading to performance improvement on Diverse-Math23K. The code and dataset is available at: https://github.com/zhouzihao501/DiverseMWP

==> rebuttal.tex <==
Review #1:

Thanks for your review. Here are the detailed responses (RA: Question A, R1: Reject reason 1, and so on).

QA_R1: Paper Focus
R1:First of all, the title of the paper seems misleading. The phrase ‘Learning from Analogy' has not been supposed by any statement in the subsequent part of the paper. Though the title talks about diverse question generation, the abstract claims to ‘... to solve MWPs by…'. The fact is the paper has intended to generate diverse questions and their effect on a solver.
QA: What is the primary focus? Developing a MWP solver or generating diverse questions for MWP
Response: 
We focus on generating diverse questions for MWP. Although most MWP papers work on designing better MWP solvers, we think high-quality data is  essential. By generating diverse questions for MWP training samples, the solver can improve its ability of learning by analogy, then boost its solving accuracy shown in Table2 and Table5. Furthermore, we propose a Group-Accuracy (line 447) metric to evaluate this ability. Moreover, Table7 illustrates the solver trained on DiverseMath23K can gain the ability of learning by analogy.
%In this paper, we propose the ability of learning by analogy is important for a solver. To show that our method improve this ability, we propose a Group-Acc(line 447) to better measure this ability. As shown in Table2 and Table5, our method can effectively improve performance of solver on Group-Acc. Further more, Table7 shows some cases that indicate solver can gain the ability of learning by analogy.
%This ability of solver can be improved by changing the solver structure or augmented the training set. Among them, the problem of data is more urgent(line 85, Yang et al.). Therefore, in this paper, we propose a novel framework to generate diverse question data. The diverse questions generation framework can be a augmentation tool to improve the learning by analogy ability of solver.

QB_R3: Details about Equation Generator
R3: The diverse equation generator module requires a more detailed treatment. The paper talks about usage of heuristic rules for implementing sub-equation and unit-based strategy. Some examples of each have been provided. But they are not adequate enough to judge the coverage of the rule set. It is suggested to put the details in more formal (e.g., algorithmic) form. How is ‘different unit' defined? Do they represent the same physical quantity (e.g., Km and m)? Or, they may represent different but related quantities (e.g., Km and m per second)?
QB: How is ‘different unit' defined? Do they represent the same physical quantity (e.g., Km and m)? Or, they may represent different but related quantities (e.g., Km and m per second)?
Response: 
We regard two absolutely identical units as the same unit, otherwise they are different. Therefore, both (km, m) and (m, m/s) are different units. Actually, we tried to relax the constrains of "same unit", which generated too many unreasonable equations and decreased performance. In the sub-equation strategy, we first formulate the original equation as a binary-tree, then extract all sub-trees as sub-equations. We will add this in revision.
%To help readers better understand the principle of equations generation and equations correspond to which type of questions, we provide examples to introduce them. In practice, for sub-equation-based, we generate equation tree of the original equation then take out each sub-tree of it to1 extract  sub-equations; for unit-based, we simply attribute two identical units to the same unit, and vice versa for different units. Therefore, both (km, m) and (m, m/s) are different units. Actually we have tried a fine-grained unit distinction, but it brought more noisy data. Thanks for your good advice, we will give a detailed description of them in the Appendix if published.

QC_R5: Same Number Interaction 
QC: In designing interaction mechanism, what happens if the same number appears multiple times? Then how is the replacement candidate selected? Also, what happens if the same number appears with two units?
R5: The question generation module is simple to understand. The interaction mechanism replaces the embeddings from scenario to equation and reverse. The replacement is based on the common occurrence of a number. What happens if the same number appears multiple times? Then how is the replacement candidate selected? Also, what happens if the same number appears with two units, e..g,, X covers 2 km in 2 hours?
Response: 
In MWP datasets, each number is replaced by an independent symbol, and all numbers in the equation are replaced by the corresponding symbol in the scenario. E.g., ‘X covers 2 km in 2 hours’ is replaced by ‘X covers n0 km in n1 hours’, then input to the encoder. The exact numbers are only used in the final calculation of answers. Thus no confusion exists between same numbers in the interaction. %So even there are same numbers in the MWP, they will be represented by different symbols in the interaction. 
%In MWP datasets, numbers are always in the form of symbols, for example, ‘X covers 2 km in 2 hours’ is ‘X covers num_0 km in num_1 hours’ and the corresponding equation is consists of num_0 and num_1 too. We preserve this form in question generator. Therefore each number in MWP is unique. %The specific number is meaningless in the embedding.

QD_R8_R10: Metric
QD: why an indirect method like using the accuracy of an existing solver was used? Why was a direct method of measuring the accuracy not adopted?
R8: As far as the performance evaluation, why an indirect method like using the accuracy of an existing solver was used? Why was a direct method of measuring the accuracy not adopted?
R10: It is not clear how the results on BLEU, ROUGE-* were computed. What is a reference string here?
Response: 
Since we don't have ground-truth for generated MWPs (scenario+question+equations), we adopt an indirect metric. As the accuracy of MWP solver is highly related to the quality of training data (Yang et al. line 85), we take this accuracy to evaluate our generated data.  
Additionally, we evaluate the quality of question generator by BLEU, BERT F1 and ROUGE-* values (Table 4), indicating its effectiveness. The question generator (one main part of our proposed DQGF) is trained on UnbiasedMWP, and BLEU and ROUGE-* are reported on test data (line 438), where questions are manually annotated (line 074) as the reference.

%we train question generator on UnbiasedMWP(line 437), the reference string is the questions in UnbiasedMWP. 
%If the solver trained on our generated data is better than that from the original data, it means these generated data is useful, indicating our diverse questions generation is effective as shown in Table 2, 5 and 7.

%Actually there is no ground-truth to directly measure the accurary of our generated data. To measure the quality of generated data, we can only adapt the performance of solvers on the diversity questions dataset. % we aim to generate diverse questions instead of a new solver, so to evalaute these data quality, we take an existing solver to evaluate the perforamnce. if it is increased, then we can say these data is useful. But we can not directly evalaute the data quality because we do not have ground -truth of these genrated data.

QE_R7: SVAMP performance
QE: Why was performance on SVAMP not reported?
R7: The primary concern that the paper seems to address is to address the limitation of shallow heuristics of the existing MWP solvers. They have Patel et al. (line 197) to support this statement. Patel et al. curated a set of hard MWP instances named as SVAMP. The existing MWP solvers performed poorly on that dataset. However, this paper did not report any results on this dataset. To my view this is the most crucial one.
Response: 
Currently, our question generator is learned from a Chinese MWP dataset. Therefore it cannot be directly applied to English datasets, e.g. SVAMP. Nonetheless, our method can be readily extended to English datasets. We verified the generated diverse questions are effective to improve the ability of learning by analogy for MWP solver, thus able to overcome the question sensitivity issue in SVAMP. 

%Our diverse questions generation model is trained on an existing Chinese MWP dataset (UnbiasedMWP, line 438). Therefore, we can not directly apply our current model in English dataset. Although we tried to utilize machine translation, the translation quality is not satisfied, so we abandon the evaluation on SVAMP. Frankly speaking, Patel et al. motivates us to do this work on generating diverse questions in MWP to improve the ability of learning by analogy of a solver, which overcomes the question sensitivity issue of SVAMP, so we believe our method will also be effective in SVAMP dataset. 
%that's why we report group-accuracy and Deq-accuracy to specifically demonstrate the effectiveness. So we believe our method will also be effective in SVAMP dataset.

%We firstly chose Chinese dataset UnbiasedMWP to train our question generator because it is better suited to our tasks. Therefore we test our method on the Chinese dataset Math23k. To address the limitation of shallow heuristics, we also evaluate the Question Sensitivity and Deq-Acc, which are proposed by Patel et al. Experiment show that the solver with our method has a huge improvement in Question Sensitivity, which is the biggest reason why other solvers perform poorly on SVAMP (Table13 in paper of SVAMP). So if solver applies our method, it can achieve the predictable improvement on SVAMP as well. %This motivates us to generate diverse questions, however, this is English.

R2: Shallow heuristics
The paper claims (line 198-202) that ‘...existing MWP solvers rely on shallow heuristics….' and the proposed framework helps to solve the issues. However, no experiments have been conducted to show how the proposed method is dealing with better heuristics. The experiments show that the diverse questions are helpful in improving MWP performance. However, I don't see any evidence that the performance improvement can be attributed to superior heuristics.
Response: In Table5, Deq-Accuracy (line 568) actually indicates the solver learns superior heuristics, the lower the better. Patel et al. identified such "shallow heuristics" issue, and proposed Deq-Accuracy to evaluate the solver on this issue. %The Deq-Accuracy reports the accuracy that a solver predicts the answer without the question, so a deep understanding solver should have lower value on this metric, because it is unreasonable to predict a correct answer if we do not have a question.  %‘MWP solvers rely on shallow heuristics’ is firstly proposed by Patel et al.(line 84), which is a research hotspot in MWP recently. They expose this phenomenon by pool performance when the question of MWP is changed or deleted(just preserve scenario). Our work make these phenomenas better. In Table 5, we can see that the solver significantly reduce the accuracy when the questions are deleted(Deq-Acc). And in other experiments, we can see that our method effectively improves the performance of solver when the questions are changed. 

 
R4_R9_R11: Diversity evaluation
R4:The most important contribution in this work is claimed to imbibe diversity, However, ‘Diverse Equations Generator' hardly talks about any method for implementing diversity. An evaluation of the equation generation module is required as it may affect the question generator module.
R9: The experimental result shows that same unit based generation brings the most benefit. But this is in contrast with the diversity objective. A clear explanation is required.
R11: The primary contribution of the paper is diverse question generation. However, no experiment measured the diversity aspect.
Response: 
We propose three strategies, each generating various equations. Such equations promote the diversity of generated questions as illustrated in Table6. Since we don't have ground-truth of the generated equations, we can't conduct direct evaluation. Instead, we compare the accuracy of the solver trained on the data from different strategies (Table3) where the same unit brings the most benefit. This is not in contrast with diversity because same-unit can cause high-quality multi-view questions such as ‘total’, ‘ratio’ or ‘comparing’ (Table6 and Appendix).
%which are input to our question generator to generate diverse questions as shown by examples in Table6. 
%We evaluate these three strategies 
%In table3, the same unit brings the most benefit. This is not in contrast with diversity because same-unit can also cause multi-view questions such as ‘total’, ‘ratio’ or ‘comparing’ (Table6 and Appendix).
 
%In fact the diversity of questions comes from the diversity of equations. To ensure the diversity of the equations, we propose sub-equation, same unit and different units method to generate equations. To evaluate the equations generator, we did an ablation experiment(Table 3) and observed generated data(Table 6). Table3 shows that each method contributes useful equations. Among them the same-unit contributes the most, it is not in contrast with diversity because same-unit can lead the multi-view questions such as ‘total’, ‘ratio’ or ‘comparing’(Table6). It’s difficult to find other objective metrics to evaluate diversity(like human evaluation is subjective).

R6: Data Quality
The use of the term ‘beam search' (line 418) in the Data Filter section is misleading. The strategy only selects the top k predicted equations. This has an underlying assumption that the predictions are ranked. However, no raking function has been defined for the predicted questions. Relying on the existing solvers for the filtering task may have undesired effect in creating a benchmark dataset like DiverseMath23, one of the contributions of the work. Thus I am bit skeptical in treating DiverseMath23 to be a benchmark dataset for MWP.
Response: 
In  Data Filter, questions are not necessary to rank. Actually, we conduct  filtering based on whether the expert solver is able to solve MWP correctly (i.e., the top k predicted answers contain the correct one, line 424-427). See General Response for the quality assurance of Diversemath23k.
%Given a generated question in the augmented MWP, we adopt one expert solver (MWP_BERT) to predict its top k equations (i.e., top k answers), if any answer can match the ground-truth answer in the augmented MWP, then we keep this MWP, otherwise it is filtered (line 424-427). 
%The quality assurance of Diversemath23k is discussed in the General Response.
%Furthermore, we manually check the generated Diversemath23k to guarantee the quality, and more details are in the General response (GR1).  
%the quality of our Diversemath23k is guaranteed by the final manual check (line 559-564). More details are in the General response (GR1). 


%The output of filter(MWP-Bert) is a equation sequence. Therefore it is not misleading, we use beam search in generating each token of equation sequence and the beam-size is k. At last we can get top k equations.
%For Diversemath23k, We are also aware of the importance of accuracy for a publicly benchmark dataset. Therefore, the validation and test sets are rigorously checked manually to ensure the completely correction and diversity for data(line 559). In details, we checked each data then fixed or deleted which are incorrect. Furthermore, we added more diverse questions to make it complete. For training set, we did a manual sample checking and found that our generated questions were also interesting and mostly correct.

%R10:
%we train question generator on UnbiasedMWP(line 437), the reference string is the questions in UnbiasedMWP.


Review #2:
QA：What is Deq-Accuracy?
Response:  Thanks. Deq-Acc is proposed by Patel el al. to evaluate Question Sensitivity, the lower the better (line 569). Concretely, it measures the accuracy that the solver predicts the answer of a MWP by DEleting Questions (i.e., only input scenario). A better solver should have higher question sensitivity, thus a lower Deq-Acc is expected. 

Review #3
R1: Data Quality
Verifying the correctness of generated questions is very challenging, it is hard to convince the readers using the MWP-BERT + beam search can give us accurate questions. As the authors mentioned the DiverseMath23k is going to be released, it would be confusing about the dataset quality. I think this is the most important problem in math word question generation.
Response: Thanks. See General Response.
%Quality assurance of Diversemath23k is done by the final manual check. More details are in the General response (GR1). 

R2: Model generalization
Though the performance is improved, I still doubt whether such improvements generalize to other datasets or larger models. For example, as UnbiasedMWP is a small dataset, also both of Unbiased MWP and math23k are Chinese datasets, We expect see more results in some datasets such as MathQA, SVAMP, GSM8k as well. Further, whether such data will be helpful for larger models is questionable, it is also important to see if the improvements would be neglectable after the model becomes larger.
Response: 

% Thanks for your suggestion. Currently, our diverse question generator is learned from a Chinese MWP dataset, so it cannot be directly applied to English MWP datasets, such as MathQA, SVAMP, GSM8k. But it is not difficult to extend our method in these English datasets, and the generated high-quality diverse questions will also be effective to improve the ability of learning by analogy for a MWP solver, which then can overcome the multi-questions issue of GSM8k and question sensitivity issue of SVAMP. 

Currently, our diverse question generator is learned from a Chinese MWP dataset. Therefore it cannot be directly applied to English datasets, e.g. SVAMP. Nonetheless, our method can be readily extended to English datasets. We believe the generated diverse questions are effective to improve the ability of learning by analogy for the MWP solver, thus able to overcome the multi-questions issue of GSM8k and the question sensitivity issue in SVAMP. 

Moreover, we believe our generated diverse MWP samples can benefit larger models. In this paper, we evaluate a mainstream strong solver (base chinese-bert-wwm), which is actually not small. As observed, our data significantly improves the solver(34.9->62.7, table2). Yang et al. pointed out the data bias is the main reason of poor performance on diverse questions for existing solvers, implying the usefulness of our method.
%if the training data of a large model lacks diversity, our method will be helpful.

%For datasets: 
%We firstly chose Chinese dataset UnbiasedMWP to train our question generator because it is better suited to our tasks. Therefore we test our method on the Chinese dataset Math23k. As shown in experiment, our approach greatly improves the Question Sensitivity of the solver, we can achieve predictable improvements on the GSM8K which is a multi-questions dataset and SVAMP which is related Question Sensitivity.
%For model:
%The large model(like bert-large) can’t reach the performance we improve. In fact, we have chosen a mainstream strong solver(base chinese-bert-wwm). The data bias proposed by Yang et al.(line 85) is the main reasons of pool performance on diverse questions for existing solvers. We can see the great improvement(34.9->62.7) of the model which apply our method in Table2. The ChatGPT maybe can achieve similar performance as us, because they have been trained on a wide variety of MWPs, our approach exactly can be used to generate such a variety of MWPs for training when the train set lacks diversity.



Review_#1_R6, Review_#3_R1:
For the quality of our Diversemath23k, we first adopt the beam-search strategy to increase the recall of our expert solver in the data filter (line 414-420), then we manually check all remained MWPs (line 559-564), which is much easier and more efficient than  complete human annotation. For the test and validation set, we rigorously check and correct each sample by ourselves, while we randomly check parts of samples in training set and found that our generated questions were also meaningful and credible (Appendix). Therefore, the quality of the final DiverseMath23K can be assured. 

%The quality of the Diversemath23k dataset is reliable. We are also aware of the importance of accuracy for a publicly benchmark dataset. Therefore, the validation and test sets are rigorously checked manually to ensure the completely correction and diversity for data(line 559). In details, we checked each data then fixed or deleted which are incorrect. Furthermore, we added more diverse questions to make it complete. For training set, we did a manual sample checking and found that our generated questions were also interesting, multi-view and mostly correct.
%Our filter can effectively filter out noisy data. To avoid bias in the expert model(MWP-Bert), we use strategies beam-search and comparing answers instead of equation sequence. Figure 3 shows the effectiveness of our filter, when beamsize is between 7 and 8 (tending to no filter) the quality of the generated data is significantly reduced. In addition, we have sampled the generated data and found that the data after filter is mostly correct and diverse.


